QuFrame: Pauli Frame Tracking for Fault-Tolerant Quantum Control

Fault-tolerant quantum computing requires continuous quantum error correction (QEC) to suppress physical noise. While Clifford-only workloads can defer corrections to software post-processing, universal computation breaks this paradigm: executing non-Clifford gates via magic-state gadgets introduces hard, real-time control-flow dependencies on error-corrected measurements. Consequently, the controller must extract syndromes, decode them, and update the Pauli frame in real time, closing the entire QEC loop within a strict $1\,\mu\text{s}$ cycle. However, prior proposals on Pauli frame tracking remain largely theoretical, leaving the microarchitectural bottlenecks of tracking, resolving, and synchronizing frame updates across distributed control pipelines unaddressed. To this end, we present QuFrame, a control microarchitecture for real-time Pauli frame tracking that closes the QEC loop within $1\,\mu\text{s}$ while sustaining QPU-rate throughput. By introducing QuFrameISA, we cleanly decouple instruction execution from continuous Pauli frame management. Execution is distributed across per-qubit Instruction Resolution Engines (IREs) that resolve instructions against the frame via a single table lookup, while a Pauli Frame Management Unit enables independent, lock-free concurrent commits. To strictly guarantee the $1\,\mu\text{s}$ deadline, QuFrame pairs an asynchronous primary decoder with an on-chip fallback decoder that resolves in $144\,\text{ns}$, natively reconciling divergent updates in hardware without degrading logical error rates.

==> algorithms/decoder.tex <==
{
\newcommand{\myfontsizealgorithms}{\fontsize{8}{8}\selectfont}
\LinesNumbered
\setlength{\parskip}{0pt}
\begin{algorithm}[!htbp]
    \myfontsizealgorithms
    \SetAlgoLined
    \DontPrintSemicolon
    \SetKwProg{Fn}{Function}{:}{}
    \newcommand\mycommfont[1]{\fontsize{8}{8}\textcolor{codegreen}{#1}}
    \SetCommentSty{mycommfont}
    \SetNoFillComment
    \underline{{\bf RunStrongDecoder}()} \\
    \Begin{
        \While{\textnormal{controller is active}}{
            \tcc{Stage 1: receive a syndrome over the link}
            $(\mathcal{S}, t_{\text{syn}}) \gets \text{ReceiveSyndromeOverLink}()$

            \tcc{Stage 2: decode, timing the call}
            $t_0 \gets \text{Now}()$; \quad $\mathbf{C}_{\text{opt}} \gets \text{StrongDecoder}(\mathcal{S})$; \quad $elapsed \gets \text{Now}() - t_0$

            \tcc{Stage 3: a decoder that misses the budget is dropped, not reconciled}
            $dropped \gets (\textnormal{cutoff} > 0) \textnormal{ and } (elapsed > \textnormal{cutoff})$

            \tcc{Stage 4: send the result back}
            $\text{SendResultOverLink}(dropped \mathbin{?} \emptyset : \mathbf{C}_{\text{opt}},\ t_{\text{syn}},\ dropped)$
        }
    }
    \BlankLine
    \underline{{\bf ReceiveResultLoop}()} \\
    \Begin{
        \While{\textnormal{controller is active}}{
            \tcc{Stage 1: receive the strong decoder's result over the link}
            $(\mathbf{C}_{\text{opt}}, t_{\text{syn}}, dropped) \gets \text{ReceiveResultOverLink}()$

            \tcc{Stage 2: pop unconditionally -- must not leak just because it is dropped}
            $\mathbf{C}_{\text{pre}} \gets \text{RetrieveFastCorrection}(t_{\text{syn}})$

            \uIf{$dropped$}{
                \tcp{too slow to trust: leave the predecoder's correction as final}
                \textbf{continue}
            }

            \tcc{Stage 3: reconcile against what the predecoder already applied}
            $\text{ReconcileResult}(\mathbf{C}_{\text{opt}}, \mathbf{C}_{\text{pre}}, t_{\text{syn}})$
        }
    }
    \BlankLine
    \underline{{\bf ApplyCorrection}(qubit: $k$, correction: $\Delta$, syndrome time: $t_{\text{syn}}$)} \\
    \Begin{
        \tcc{Stage 1: commute the correction through history and commit}
        \Repeat{ok}{
            $(P,v,t) \gets \text{ReadFrame}(k)$

            \tcp{note down all the qubits affected by 2q gates}
            $\mathbf{C} \gets \text{CommuteThroughHistory}(\Delta,k,t_{\text{syn}},t)$

            \tcp{always single-component: a correction is $X$-only or $Z$-only (\S\ref{design:sync})}
            $ok \gets \text{TryCommit}(k,v,P \oplus \mathbf{C}[k])$
        }

        \tcc{Stage 2: apply any spillover}
        \ForEach{$q \in \textnormal{Keys}(\mathbf{C}) \setminus \{k\}$}{$\text{ApplyDirect}(q,\mathbf{C}[q])$}
    }
    \BlankLine
    \underline{{\bf ReconcileResult}(optimal: $\mathbf{C}_{\text{opt}}$, predecoder: $\mathbf{C}_{\text{pre}}$, time: $t_{\text{syn}}$)} \\
    \Begin{
        \tcc{Stage 1: XOR delta over the union of both corrections' qubits}
        $\mathbf{C}_{\text{delta}} \gets \mathbf{C}_{\text{opt}} \oplus \mathbf{C}_{\text{pre}}$

        \tcc{Stage 2: apply only the difference}
        \ForEach{$q \in \textnormal{Keys}(\mathbf{C}_{\text{delta}})$ \textnormal{where} $\mathbf{C}_{\text{delta}}[q] \neq I$}{$\text{ApplyCorrection}(q, \mathbf{C}_{\text{delta}}[q], t_{\text{syn}})$}
    }
    \caption{The remote strong decoder and result reconciliation (\S\ref{decoder}).}
    \label{alg:globaldecoder}
\end{algorithm}
}


==> algorithms/ire.tex <==
{
\newcommand{\myfontsizealgorithms}{\fontsize{8}{8}\selectfont}
\LinesNumbered
\setlength{\parskip}{0pt}
\begin{algorithm}[!htbp]
    \myfontsizealgorithms
    \SetAlgoLined
    \DontPrintSemicolon
    \SetKwProg{Fn}{Function}{:}{}
    \newcommand\mycommfont[1]{\fontsize{8}{8}\textcolor{codegreen}{#1}}
    \SetCommentSty{mycommfont}
    \SetNoFillComment
    
    % \underline{{\bf ExecuteQubitProgram}(qubit: $i$)} \\
    % \Begin{
    %     \While{\textnormal{controller is active}}{
    %         \tcc{Stage 1: fetch the next instruction}
    %         $inst \gets$ \text{NextInstruction}($i$)
    %
    %         \tcc{Stage 2: control-flow instructions never touch the frame}
    %         \uIf{$inst$ \textnormal{ends program}}{\textbf{break}}
    %         \uElseIf{$inst$ \textnormal{is a barrier}}{
    %             \text{ArriveAtBarrier}()
    %
    %             \textbf{continue}
    %         }
    %         \uElseIf{$inst$ \textnormal{has partner} $j$ \textnormal{with} $i > j$}{
    %             \text{WaitForPartner}($i, inst$)
    %
    %             \textbf{continue}
    %         }
    %
    %         \tcc{Stage 3: resolve against the frame, retrying as needed}
    %         $out \gets$ \text{ResolveAndCommit}($i, inst$)
    %
    %         \tcc{Stage 4: forward pulse if needed}
    %         \If{$out$ \textnormal{needs a pulse}}{\text{ForwardPulse}($out$)}
    %     }
    % }
    % \BlankLine
    
    \underline{{\bf ResolveAndCommit}(qubit: $i$, instruction: $inst$)} \\
    \Begin{
        \uIf{$inst$ \textnormal{has partner} $j$}{
            \Repeat{$ok_i \textnormal{ and } ok_j$}{
                \tcc{Stage 1: read both rows and resolve}
                $(P_i,v_i) \gets \text{ReadFrame}(i)$
                
                $(P_j,v_j) \gets \text{ReadFrame}(j)$

                $(P_i',P_j',out) \gets \text{ResolveTwoQubit}(P_i,P_j,inst)$

                \tcc{Stage 2: commit both rows independently}
                $ok_i \gets \text{TryCommit}(i,v_i,P_i')$

                $ok_j \gets ok_i \textnormal{ and } \text{TryCommit}(j,v_j,P_j')$

                \If{$ok_i$ \textnormal{and not} $ok_j$}{
                    \tcp{undo our own commit}
                    \text{Rollback}($i, P_i' \oplus P_i$)

                    $ok_i \gets \textbf{false}$
                }
            }
        }
        \Else{
            \Repeat{ok}{
                \tcc{Stage 1: read the row and resolve}
                $(P_i,v_i) \gets \text{ReadFrame}(i)$
                
                $(P_i',out) \gets \text{Resolve}(P_i,inst)$
                \tcc{Stage 2: commit via a single row-level CAS}
                $ok \gets \text{TryCommit}(i,v_i,P_i')$
            }
        }
        \Return{$out$}
    }
    \caption{The workflow of the instruction resolver (\S\ref{ire}).}
    \label{alg:ire}
\end{algorithm}
}

==> algorithms/predecoder.tex <==
{
\newcommand{\myfontsizealgorithms}{\fontsize{8}{8}\selectfont}
\LinesNumbered
\setlength{\parskip}{0pt}
\begin{algorithm}[!htbp]
    \myfontsizealgorithms
    \SetAlgoLined
    \SetKwProg{Fn}{Function}{:}{}
    \newcommand\mycommfont[1]{\fontsize{8}{8}\textcolor{codegreen}{#1}}
    \SetCommentSty{mycommfont}
    \SetNoFillComment
    \underline{{\bf RunFastDecoder}()} \\
    \Begin{
        \While{\textnormal{controller is active}}{
            $(\mathcal{S}, t_{\text{syn}}) \gets$ \text{WaitForSyndrome}() \tcp*[r]{co-located, in-process -- no added latency (\S\ref{design:decoder-interface})}
            $\mathbf{C}_{\text{fast}} \gets$ \text{FastDecoder}($\mathcal{S}$) \;
            \text{RecordFastCorrection}($t_{\text{syn}}, \mathbf{C}_{\text{fast}}$) \tcp*[r]{logged for later reconciliation, Algorithm~\ref{alg:globaldecoder}}
            \ForEach{$q \in \textnormal{Keys}(\mathbf{C}_{\text{fast}})$ \textnormal{where} $\mathbf{C}_{\text{fast}}[q] \neq \textnormal{identity}$}{
                \text{ApplyCorrection}($q, \mathbf{C}_{\text{fast}}[q], t_{\text{syn}}$) \tcp*[r]{shared with the strong decoder, Algorithm~\ref{alg:globaldecoder}}
            }
        }
    }
    \caption{The local fast predecoder.}
    \label{alg:predecoder}
\end{algorithm}
}


==> figures/lifetime.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/pdfs/lifetime.pdf}
    \caption{Lifetime of a QEC-protected application. \emph{This work covers elements marked in green.}}
    \label{fig:lifetime}
\end{figure}

==> figures/motivation_ire.tex <==
 \begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/pdfs/motivation_ire.pdf}
    \caption{Change in Pauli frame state based on applied quantum instruction. \emph{CNOT gates cause X errors to spread to target qubits.}}
    \label{fig:motivation_ire}
\end{figure} 

==> figures/motivation_sync.tex <==
 \begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/pdfs/motivation_sync.pdf}
    \caption{Two independent cores may execute gates with different speed. \emph{Executing CNOT\_TARGET before H gate can lead to incorrect Pauli frame.}}
    \label{fig:motivation_sync}
\end{figure} 

==> plots/buffer_eval.tex <==
\begin{figure*} [t]
    \centering
    \includegraphics[width=0.9\linewidth]{plots/pdfs/controller_eval_buffer.pdf}
    \caption{Op-history buffer analysis. \emph{a) Logical error rate with and without the op-history buffer, per decoding configuration. b) Logical error rate vs. buffer size. c) Predecoder path latency vs. buffer size. d) Memory cost of the op-history buffer.}}
    \label{fig:buffer_eval}
\end{figure*}


==> plots/decoding_time.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{plots/pdfs/pymatching_decode_time_distribution_100k.pdf}
    \caption{Decoding latency distribution for PyMatching~\cite{higgott2021pymatchingpythonpackagedecoding}. \emph{Measured across 100000 batch-executed shots for a distance-17 surface code (17 rounds) under depolarizing noise (p=0.001).}}
    \label{fig:decoding_time}
\end{figure}

==> plots/fallback_decoder.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{plots/pdfs/fallback_decoder.pdf}
    \caption{Fallback decoder across code distance. \emph{a) Logical error rate of the three decoding configurations. b) Latency of the deployed path against the external decoder. c) Memory footprint of both decoders.}}
    \label{fig:fallback}
\end{figure*}


==> plots/flushing_impact.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{plots/pdfs/pre_t_correction_depolarizing_disproportion_overhead.pdf}
    \caption{Impact of flushing the Pauli frame on logical error rate. \emph{Estimated based on frequency of T-gates in qft quantum circuit protected with surface code (d=5) with depolarizing noise model (p=0.001) ran for 60000 shots.}}
    \label{fig:flushing}
\end{figure}

==> plots/latency_eval.tex <==
\begin{figure*} [t]
    \centering
    \includegraphics[width=0.9\linewidth]{plots/pdfs/controller_eval_latency.pdf}
    \caption{Latency analysis. \emph{a) Per-gate dispatch overhead vs.\ QubiC 2.0. b) Latency of both decode paths across code distance. c) Predecoder- and decoder-path budget breakdowns. d) Logical error rate of the three decoding configurations across code distance.}}
    \label{fig:latency_eval}
\end{figure*}


==> plots/ler_eval.tex <==
\begin{figure*} [t]
    \centering
    \includegraphics[width=0.9\linewidth]{plots/pdfs/controller_eval_ler_memory.pdf}
    \caption{Logical error rate and predecoder analysis. \emph{a) Logical error rate of \projecttitle{} vs. a zero-latency ideal, across physical error rate. b) Logical error rate of the three decoding configurations at d=5. c) The same three configurations across code distance. d) Memory cost of both decode paths across code distance.}}
    \label{fig:ler_eval}
\end{figure*}


==> plots/lock_approach.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{plots/pdfs/controller_eval_frame_split_gatemix.pdf}
    \caption{Throughput and memory utilization, combined vs.\ split Pauli Frame Table, as the contending workload's basis-changing (joint-update) fraction varies. Split wins below $\sim$50\% and real circuits sit near 11\%; combined wins only once joint updates dominate.}
    \label{fig:lock_split}
\end{figure}


==> plots/scalability_eval.tex <==
\begin{figure*} [t]
    \centering
    \includegraphics[width=0.9\linewidth]{plots/pdfs/controller_eval_rq6_7.pdf}
    \caption{Scalability analysis. \emph{a) Memory vs. number of qubits and gate set. b) Resolution time vs. number of qubits and gate set. c) Memory of both decode paths across code distance. d) Memory of the safe vs. unsafe Pauli Frame Table.}}
    \label{fig:scalability_eval}
\end{figure*}


==> plots/sync_buffer.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{plots/pdfs/sync_buffer.pdf}
    \caption{Synchronization and op-history ablations. \emph{a) Frame table throughput vs.\ contending cores, with and without synchronization. b) Logical error rate vs.\ op-history length at two distances. c) Fallback decode path latency vs.\ op-history length. d) Op-history memory vs.\ number of qubits, per ring length.}}
    \label{fig:sync_buffer}
\end{figure*}


==> plots/sync_eval.tex <==
\begin{figure*} [t]
    \centering
    \includegraphics[width=0.9\linewidth]{plots/pdfs/controller_eval_sync.pdf}
    \caption{Op-history buffer analysis. \emph{a) Memory of the safe vs. unsafe Pauli Frame Table. b) Logical error rate without the op-history buffer and across buffer sizes. c) Predecoder path latency vs. buffer size. d) Memory cost of the op-history buffer.}}
    \label{fig:sync_eval}
\end{figure*}


==> sections/acks.tex <==
%\section*{Acknowledgments}
%This work is funded by the Bavarian State Ministry of Science and the Arts as part of the Munich Quantum Valley (MQV), grant number XXX.

==> sections/design.tex <==
\section{Design}
\label{design}


\projecttitle{}'s design follows directly from the three challenges in \S\ref{motivation:challenges}. We present it by mechanism: the Assembler compilation pass that lowers the circuit into our dedicated ISA (\S\ref{design:assembler}); the Instruction Resolution Engine that performs the frame updates per qubit (\S\ref{ire}); the decentralized synchronization protocol that lets every IRE and both decoder paths share the frame table without a central bottleneck (\S\ref{design:sync}); and the decoder interface that reconciles a fast, approximate correction against a slower, more accurate one without ever blocking the IRE (\S\ref{design:decoder-interface}).




==> sections/methodology.tex <==
\section{Methodology}
\label{methodology}

% --- ORIGINAL TEXT AND NOTES ---
% \section{Methodology}
% -------------------------------

[Placeholder: Describe the experimental methodology, similar to the "paper pinball" approach. Detail how the system is modeled or simulated if not fully run on live quantum hardware.]

\subsection{Workloads}
[Placeholder: Detail the benchmarks used, e.g., factor247\_n15, bwt\_n37, feynman, toffoli\_n3.]

\subsection{Metrics}
[Placeholder: Define the key metrics used to evaluate the system, such as reduction in stall cycles, total execution time, and logical error rates.]

==> tables/ibm_heron_lut.tex <==
\begin{table*}[t]
\centering
\caption{Example with IBM Heron gate set.}
\label{tab:heron_optimization_lut}
\footnotesize
\begin{tabularx}{\textwidth}{p{2.9cm} c c X}
\toprule
\textbf{QuFrameISA instruction} & \textbf{Frame in} & \textbf{Frame out} & \textbf{Heron-native realization} \\ \midrule
$\sqrt{X}$ (native single-qubit gate) & $(X_F, Z_F)$ & $(X_F \oplus Z_F,\, Z_F)$ & \texttt{pulse\_id} indexes one calibrated $\sqrt{X}$ pulse, dispatched unconditionally; the frame update is the same kind of Clifford conjugation as $H$/$S$ in Table~\ref{tab:clifford_ire_lut} -- no dependence on frame in the pulse itself. \\ \addlinespace
$R_z(\theta)$ (virtual-$Z$) & $(X_F, Z_F)$ & $(X_F, Z_F)$ & Implemented as a zero-duration phase update to the qubit's local drive frame, not a physical pulse; frame is unaffected, since a $Z$-rotation commutes with every Pauli tracked here up to the untracked global sign. \\ \addlinespace
$\mathrm{CNOT}$ & \multicolumn{2}{c}{as Table~\ref{tab:clifford_ire_lut}} & Decomposed to Heron's native CZ plus single-qubit frame conjugation once, at compile time; \texttt{LUT.RESOLVE2}'s conjugation math is unchanged, only the \texttt{pulse\_id} it dispatches differs from a directly-CNOT-native backend. \\ \addlinespace
$\mathrm{CZ}(A,B)$ (native two-qubit gate) & \makecell{$(X_A,Z_A)$\\$\otimes(X_B,Z_B)$} & \makecell{$(X_A,\,Z_A\oplus X_B)$\\$\otimes(X_B,\,Z_B\oplus X_A)$} & Dispatched directly as one \texttt{pulse\_id}, unconditionally; identical conjugation rule to Table~\ref{tab:clifford_ire_lut}'s backend-agnostic CZ row. \\ \addlinespace
$T, T^\dagger$ (magic-state gadget) & $(X_F, Z_F)$ & $(X_F,Z_F)\oplus\mathrm{Byproduct}(X_F,Z_F,m)$ & Fixed CZ-with-ancilla-plus-measurement sequence, dispatched unconditionally and identically regardless of frame; \texttt{byproduct\_table\_base} indexes 8 pre-synthesized classical resolution rules (4 incoming frames $\times$ 2 ancilla outcomes) applied to the measurement outcome $m$ once it returns -- no Heron-specific control logic beyond the ordinary CZ pulse above. \\
\bottomrule
\end{tabularx}
\end{table*}

